On the multipliers at fixed points of self-maps of the projective plane

This paper deals with holomorphic self-maps of the complex projective plane and the algebraic relations among the eigenvalues of the derivatives at the fixed points. These eigenvalues are constrained by certain index theorems such as the holomorphic Lefschetz fixed-point theorem. A simple dimensional argument suggests there must exist even more algebraic relations that the ones currently known. In this work we analyze the case of quadratic self-maps having an invariant line and obtain all such relations. We also prove that a generic quadratic self-map with an invariant line is completely determined, up to linear equivalence, by the collection of these eigenvalues. Under the natural correspondence between quadratic rational maps of $\mathbb{P}^2$ and quadratic homogeneous vector fields on $\mathbb{C}^3$, the algebraic relations among multipliers translate to algebraic relations among the Kowalevski exponents of a vector field. As an application of our results, we describe the sets of integers that appear as the Kowalevski exponents of a class of quadratic homogeneous vector fields on $\mathbb{C}^3$ having exclusively single-valued solutions.

==> multipliers <==
@article {ramirez-twin,
    AUTHOR = {Ram\'{\i}rez, Valente},
     TITLE = {Twin vector fields and independence of spectra for quadratic
              vector fields},
   JOURNAL = {J. Dyn. Control Syst.},
  FJOURNAL = {Journal of Dynamical and Control Systems},
    VOLUME = {23},
      YEAR = {2017},
    NUMBER = {3},
     PAGES = {623--633},
      ISSN = {1079-2724},
   MRCLASS = {37F75 (32M25 32S65)},
  MRNUMBER = {3657280},
 ZBLNUMBER = {1381.37058},
       DOI = {10.1007/s10883-016-9344-5},
       URL = {https://doi.org/10.1007/s10883-016-9344-5},
}


@article{Kudryashov-R,
    AUTHOR = {Kudryashov, {Yu}ry and Ram\'{i}rez, Valente},
     TITLE = {Spectra of quadratic vector fields on $\mathbb{C}^2$: The missing relation},
      NOTE = {Preprint arXiv:1705.06340 [math.CV]},
      YEAR = {2018},
       URL = {http://arxiv.org/abs/1705.06340},
}


@article{ramirez2016woods,
    AUTHOR = {Ram\'{i}rez, Valente},
     TITLE = {The {W}oods {H}ole trace formula and indices for vector fields and foliations on $\mathbb{C}^{2}$},
      NOTE = {Preprint arXiv:1705.1608.05321 [math.CV]},
      YEAR = {2016},
       URL = {http://arxiv.org/abs/1608.05321},
}


@article {guillot-pointfixe,
    AUTHOR = {Guillot, Adolfo},
     TITLE = {Un th\'eor\`eme de point fixe pour les endomorphismes de l'espace
              projectif avec des applications aux feuilletages alg\'ebriques},
   JOURNAL = {Bull. Braz. Math. Soc. (N.S.)},
  FJOURNAL = {Bulletin of the Brazilian Mathematical Society. New Series.
              Boletim da Sociedade Brasileira de Matem\'atica},
    VOLUME = {35},
      YEAR = {2004},
    NUMBER = {3},
     PAGES = {345--362},
      ISSN = {1678-7544},
   MRCLASS = {32S65 (57R25 57R30)},
  MRNUMBER = {2106309},
 ZBLNUMBER = {1085.58007},
MRREVIEWER = {M. G. Soares},
       DOI = {10.1007/s00574-004-0018-7},
       URL = {https://doi.org/10.1007/s00574-004-0018-7},
}


@article {guillot-semi,
    AUTHOR = {Guillot, Adolfo},
     TITLE = {Semicompleteness of homogeneous quadratic vector fields},
   JOURNAL = {Ann. Inst. Fourier (Grenoble)},
  FJOURNAL = {Universit\'e de Grenoble. Annales de l'Institut Fourier},
    VOLUME = {56},
      YEAR = {2006},
    NUMBER = {5},
     PAGES = {1583--1615},
      ISSN = {0373-0956},
   MRCLASS = {32S65 (34M05 34M35 37F75)},
  MRNUMBER = {2273865},
 ZBLNUMBER = {1110.37040},
MRREVIEWER = {Bruno A. Sc\'ardua},
       DOI = {10.5802/aif.2221},
       URL = {http://aif.cedram.org/item?id=AIF_2006__56_5_1583_0},
}


@article {guillot-chazy,
    AUTHOR = {Guillot, Adolfo},
     TITLE = {The geometry of {C}hazy's homogeneous third-order differential
              equations},
   JOURNAL = {Funkcial. Ekvac.},
  FJOURNAL = {Funkcialaj Ekvacioj. Serio Internacia},
    VOLUME = {55},
      YEAR = {2012},
    NUMBER = {1},
     PAGES = {67--87},
      ISSN = {0532-8721},
   MRCLASS = {34M55 (32M25 32S65)},
  MRNUMBER = {2976043},
 ZBLNUMBER = {1251.34102},
MRREVIEWER = {Jes\'us Muci\~no-Raymundo},
       DOI = {10.1619/fesi.55.67},
       URL = {https://doi.org/10.1619/fesi.55.67},
}

@article {guillot-rebelo,
    AUTHOR = {Guillot, Adolfo and Rebelo, Julio},
     TITLE = {Semicomplete meromorphic vector fields on complex surfaces},
   JOURNAL = {J. Reine Angew. Math.},
  FJOURNAL = {Journal f\"ur die Reine und Angewandte Mathematik. [Crelle's
              Journal]},
    VOLUME = {667},
      YEAR = {2012},
     PAGES = {27--65},
      ISSN = {0075-4102},
   MRCLASS = {37F75 (32M25 32S65)},
  MRNUMBER = {2929671},
 ZBLNUMBER = {1250.32023},
MRREVIEWER = {Filippo Bracci},
       DOI = {10.1515/CRELLE.2011.127},
}

@article {guillot-qc3,
    AUTHOR = {Guillot, Adolfo},
     TITLE = {Quadratic differential equations in three variables without
              multivalued solutions: {P}art {I}},
   JOURNAL = {SIGMA Symmetry Integrability Geom. Methods Appl.},
  FJOURNAL = {SIGMA. Symmetry, Integrability and Geometry. Methods and
              Applications},
    VOLUME = {14},
      YEAR = {2018},
     PAGES = {122, 46 pages},
      ISSN = {1815-0659},
   MRCLASS = {34M55 (34M35 34M45)},
  MRNUMBER = {3874674},
       DOI = {10.3842/SIGMA.2018.122},
       URL = {https://doi.org/10.3842/SIGMA.2018.122},
}

@article {mattuck,
    AUTHOR = {Mattuck, Arthur},
     TITLE = {The field of multisymmetric functions},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {19},
      YEAR = {1968},
     PAGES = {764--765},
      ISSN = {0002-9939},
   MRCLASS = {14.01},
  MRNUMBER = {0225774},
 ZBLNUMBER = {0159.05303},
MRREVIEWER = {R. Jacobowitz},
       DOI = {10.2307/2035879},
       URL = {http://dx.doi.org/10.2307/2035879},
}


@book {GKZ,
    AUTHOR = {Gelfand, I. M. and Kapranov, M. M. and Zelevinsky, A. V.},
     TITLE = {Discriminants, resultants, and multidimensional determinants},
    SERIES = {Mathematics: Theory \& Applications},
 PUBLISHER = {Birkh\"auser Boston, Inc., Boston, MA},
      YEAR = {1994},
     PAGES = {x+523},
      ISBN = {0-8176-3660-9},
   MRCLASS = {14N05 (13D25 14M25 15A69 33C70 52B20)},
  MRNUMBER = {1264417},
 ZBLNUMBER = {0827.14036},
MRREVIEWER = {I. Dolgachev},
       DOI = {10.1007/978-0-8176-4771-1},
       URL = {http://dx.doi.org/10.1007/978-0-8176-4771-1},
}


@book {GH,
    AUTHOR = {Griffiths, Phillip and Harris, Joseph},
     TITLE = {Principles of algebraic geometry},
    SERIES = {Wiley Classics Library},
      NOTE = {Reprint of the 1978 original},
 PUBLISHER = {John Wiley \& Sons, Inc., New York},
      YEAR = {1994},
     PAGES = {xiv+813},
      ISBN = {0-471-05059-8},
   MRCLASS = {14-01},
  MRNUMBER = {1288523},
 ZBLNUMBER = {0836.14001},
       DOI = {10.1002/9781118032527},
       URL = {https://doi-org.proxy.library.cornell.edu/10.1002/9781118032527},
}


@article {goriely,
    AUTHOR = {Goriely, A.},
     TITLE = {A brief history of {K}ovalevskaya exponents and modern
              developments},
      NOTE = {Sophia Kovalevskaya to the 150th anniversary},
   JOURNAL = {Regul. Chaotic Dyn.},
  FJOURNAL = {Regular \& Chaotic Dynamics. International Scientific Journal},
    VOLUME = {5},
      YEAR = {2000},
    NUMBER = {1},
     PAGES = {3--15},
      ISSN = {1560-3547},
   MRCLASS = {34D08 (34C99 37J30)},
  MRNUMBER = {1784726},
 ZBLNUMBER = {0947.37031},
       DOI = {10.1070/rd2000v005n01ABEH000120},
       URL = {https://doi.org/10.1070/rd2000v005n01ABEH000120},
}


@article {chazy,
    AUTHOR = {Chazy, Jean},
     TITLE = {Sur les \'equations diff\'erentielles du troisi\`eme ordre et
              d'ordre sup\'erieur dont l'int\'egrale g\'en\'erale a ses points
              critiques fixes},
   JOURNAL = {Acta Math.},
  FJOURNAL = {Acta Mathematica},
    VOLUME = {34},
      YEAR = {1911},
    NUMBER = {1},
     PAGES = {317--385},
      ISSN = {0001-5962},
   MRCLASS = {DML},
  MRNUMBER = {1555070},
 ZBLNUMBER = {42.0340.03},
       DOI = {10.1007/BF02393131},
       URL = {https://doi.org/10.1007/BF02393131},
}


@article {cosgrove-p2,
    AUTHOR = {Cosgrove, Christopher M.},
     TITLE = {Higher-order {P}ainlev\'e equations in the polynomial class.
              {I}. {B}ureau symbol {$\mathrm{P2}$}},
   JOURNAL = {Stud. Appl. Math.},
  FJOURNAL = {Studies in Applied Mathematics},
    VOLUME = {104},
      YEAR = {2000},
    NUMBER = {1},
     PAGES = {1--65},
      ISSN = {0022-2526},
   MRCLASS = {34M55 (34A05 37K10)},
  MRNUMBER = {1738749},
 ZBLNUMBER = {1136.34350},
MRREVIEWER = {Andrei A. Kapaev},
       DOI = {10.1111/1467-9590.00130},
       URL = {https://doi.org/10.1111/1467-9590.00130},
}


@article {ab-ii,
    AUTHOR = {Atiyah, Michael F. and Bott, Raoul},
     TITLE = {A {L}efschetz fixed point formula for elliptic complexes.
              {II}. {A}pplications},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {88},
      YEAR = {1968},
     PAGES = {451--491},
      ISSN = {0003-486X},
   MRCLASS = {57.50},
  MRNUMBER = {0232406},
 ZBLNUMBER = {0167.21703},
MRREVIEWER = {R. S. Palais},
       DOI = {10.2307/1970721},
       URL = {https://doi.org/10.2307/1970721},
}


@incollection {Ueda1994,
    AUTHOR = {Ueda, Tetsuo},
     TITLE = {Complex dynamics on projective spaces---index formula for
              fixed points},
 BOOKTITLE = {Dynamical systems and chaos, {V}ol. 1 ({H}achioji, 1994)},
     PAGES = {252--259},
 PUBLISHER = {World Sci. Publ., River Edge, NJ},
      YEAR = {1995},
   MRCLASS = {32H50},
  MRNUMBER = {1479941},
 ZBLNUMBER = {0991.32504},
MRREVIEWER = {Marco Abate},
       DOI = {10.1142/9789814536165},
}


@incollection {Abate2014,
    AUTHOR = {Abate, Marco},
     TITLE = {Index theorems for meromorphic self-maps of the projective
              space},
 BOOKTITLE = {Frontiers in complex dynamics},
    SERIES = {Princeton Math. Ser.},
    VOLUME = {51},
     PAGES = {451--462},
 PUBLISHER = {Princeton Univ. Press, Princeton, NJ},
      YEAR = {2014},
   MRCLASS = {32H50 (37B30 37F10)},
  MRNUMBER = {3289918},
 ZBLNUMBER = {1345.37042},
       DOI = {10.1515/9781400851317-018},
MRREVIEWER = {Feng Rong},
}


@incollection {Baum-Bott,
    AUTHOR = {Baum, Paul F. and Bott, Raoul},
     TITLE = {On the zeros of meromorphic vector-fields},
 BOOKTITLE = {Essays on {T}opology and {R}elated {T}opics ({M}\'emoires d\'edi\'es
              \`a {G}eorges de {R}ham)},
     PAGES = {29--47},
 PUBLISHER = {Springer, New York},
      YEAR = {1970},
   MRCLASS = {57.60 (32.00)},
  MRNUMBER = {0261635},
 ZBLNUMBER = {0193.52201},
       DOI = {10.1007/978-3-642-49197-9_4},
MRREVIEWER = {H. Suzuki},
}


@article {Camacho-Sad,
    AUTHOR = {Camacho, C\'esar and Sad, Paulo},
     TITLE = {Invariant varieties through singularities of holomorphic
              vector fields},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {115},
      YEAR = {1982},
    NUMBER = {3},
     PAGES = {579--595},
      ISSN = {0003-486X},
   MRCLASS = {58F18 (57R99 58A17 58F14)},
  MRNUMBER = {657239},
 ZBLNUMBER = {0503.32007},
MRREVIEWER = {Robert Roussarie},
       DOI = {10.2307/2007013},
       URL = {https://doi.org/10.2307/2007013},
}


@article {linsneto240,
    AUTHOR = {Lins Neto, Alcides},
     TITLE = {Fibers of the {B}aum-{B}ott map for foliations of degree two
              on {${\mathbb P}^2$}},
   JOURNAL = {Bull. Braz. Math. Soc. (N.S.)},
  FJOURNAL = {Bulletin of the Brazilian Mathematical Society. New Series.
              Boletim da Sociedade Brasileira de Matem\'atica},
    VOLUME = {43},
      YEAR = {2012},
    NUMBER = {1},
     PAGES = {129--169},
      ISSN = {1678-7544},
   MRCLASS = {37F75 (34M15)},
  MRNUMBER = {2909926},
 ZBLNUMBER = {1347.37093},
       DOI = {10.1007/s00574-012-0008-0},
       URL = {https://doi.org/10.1007/s00574-012-0008-0},
}


@article {painleve,
    AUTHOR = {Painlev\'e, P.},
     TITLE = {M\'emoire sur les \'equations diff\'erentielles dont l'int\'egrale
              g\'en\'erale est uniforme},
   JOURNAL = {Bull. Soc. Math. France},
  FJOURNAL = {Bulletin de la Soci\'et\'e Math\'ematique de France},
    VOLUME = {28},
      YEAR = {1900},
     PAGES = {201--261},
      ISSN = {0037-9484},
   MRCLASS = {DML},
  MRNUMBER = {1504376},
 ZBLNUMBER = {31.0337.03},
       DOI = {10.24033/bsmf.633},
       URL = {http://www.numdam.org/item?id=BSMF_1900__28__201_0},
}

@article {obrian,
    AUTHOR = {O'Brian, N. R.},
     TITLE = {Zeroes of holomorphic vector fields and {G}rothendieck duality
              theory},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {229},
      YEAR = {1977},
     PAGES = {289--306},
      ISSN = {0002-9947},
   MRCLASS = {58G10 (32L05)},
  MRNUMBER = {0445562},
 ZBLNUMBER = {0321.57013},
MRREVIEWER = {Yue Lin L. Tong},
       DOI = {10.2307/1998512},
       URL = {https://doi.org/10.2307/1998512},
}



@book {milnor-one,
    AUTHOR = {Milnor, John},
     TITLE = {Dynamics in one complex variable},
    SERIES = {Annals of Mathematics Studies},
    VOLUME = {160},
   EDITION = {Third},
 PUBLISHER = {Princeton University Press, Princeton, NJ},
      YEAR = {2006},
     PAGES = {viii+304},
      ISBN = {978-0-691-12488-9; 0-691-12488-4},
   MRCLASS = {37Fxx (30-01 30D05 37-01)},
  MRNUMBER = {2193309},
 ZBLNUMBER = {1281.37001},
       URL = {https://www.degruyter.com/view/product/451239},
}

@article {milnor-quad,
    AUTHOR = {Milnor, John},
     TITLE = {Geometry and dynamics of quadratic rational maps},
      NOTE = {With an appendix by the author and Lei Tan},
   JOURNAL = {Experiment. Math.},
  FJOURNAL = {Experimental Mathematics},
    VOLUME = {2},
      YEAR = {1993},
    NUMBER = {1},
     PAGES = {37--83},
      ISSN = {1058-6458},
   MRCLASS = {58F20 (30D05 32S70 58F23)},
  MRNUMBER = {1246482},
MRREVIEWER = {J. S. Joel},
 ZBLNUMBER = {0922.58062},
       DOI = {10.1080/10586458.1993.10504267},
       URL = {http://projecteuclid.org/euclid.em/1062620736},
}


@article {fujimura,
    AUTHOR = {Fujimura, Masayo},
     TITLE = {The moduli space of rational maps and surjectivity of
              multiplier representation},
   JOURNAL = {Comput. Methods Funct. Theory},
  FJOURNAL = {Computational Methods and Function Theory},
    VOLUME = {7},
      YEAR = {2007},
    NUMBER = {2},
     PAGES = {345--360},
      ISSN = {1617-9447},
   MRCLASS = {30E20 (37C25 37F10)},
  MRNUMBER = {2376676},
 ZBLNUMBER = {1151.30002},
       DOI = {10.1007/BF03321649},
       URL = {https://doi.org/10.1007/BF03321649},
}

@article {milnor-cubic,
    AUTHOR = {Milnor, John},
     TITLE = {Remarks on iterated cubic maps},
   JOURNAL = {Experiment. Math.},
  FJOURNAL = {Experimental Mathematics},
    VOLUME = {1},
      YEAR = {1992},
    NUMBER = {1},
     PAGES = {5--24},
      ISSN = {1058-6458},
   MRCLASS = {58F08 (30D05 58F23)},
  MRNUMBER = {1181083},
MRREVIEWER = {Tim Bedford},
 ZBLNUMBER = {0762.58018},
       URL = {http://projecteuclid.org/euclid.em/1048709112},
}


@article {fatou,
    AUTHOR = {Fatou, Pierre},
     TITLE = {Sur les substitutions rationnelles},
   JOURNAL = {{C. R. Acad. Sci., Paris}},
  FJOURNAL = {Comptes Rendus Hebdomadaires des Sc\'eances de l'Acad\'emie des Sciences},
      ISSN = {0001-4036},
 PUBLISHER = {Gauthier-Villars, Paris},
    VOLUME = {165},
      YEAR = {1917},
     PAGES = {992--995},
 ZBLNUMBER = {46.0520.01},
       URL = {https://gallica.bnf.fr/ark:/12148/bpt6k3118k.f992},
}


@article {julia,
    AUTHOR = {Julia, Gaston},
     TITLE = {Sur les substitutions rationnelles},
   JOURNAL = {{C. R. Acad. Sci., Paris}},
  FJOURNAL = {Comptes Rendus Hebdomadaires des Sc\'eances de l'Acad\'emie des Sciences},
      ISSN = {0001-4036},
 PUBLISHER = {Gauthier-Villars, Paris},
    VOLUME = {165},
      YEAR = {1917},
     PAGES = {1098--1100},
 ZBLNUMBER = {46.0520.02},
       URL = {http://gallica.bnf.fr/ark:/12148/bpt6k3118k.f1098},
}

@book {audin,
    AUTHOR = {Audin, Mich\`ele},
     TITLE = {Fatou, {J}ulia, {M}ontel},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {2014},
      NOTE = {The {G}reat {P}rize of {M}athematical {S}ciences of 1918, and beyond,
              Translated from the 2009 {F}rench original by the author,
              History of Mathematics Subseries},
 PUBLISHER = {Springer, Heidelberg},
      YEAR = {2011},
     PAGES = {viii+332},
      ISBN = {978-3-642-17853-5},
   MRCLASS = {01A60 (30D05 37-03 37F10)},
  MRNUMBER = {2768955},
 ZBLNUMBER = {1211.01007},
       DOI = {10.1007/978-3-642-17854-2},
       URL = {https://doi.org/10.1007/978-3-642-17854-2},
}

@article {fatou-memoire,
    AUTHOR = {Fatou, Pierre},
     TITLE = {Sur les \'equations fonctionnelles},
   JOURNAL = {Bull. Soc. Math. France },
  FJOURNAL = {Bulletin de la Soci\'et\'e Math\'ematique de France},
      ISSN = {0037-9484; 2102-622X/e},
 PUBLISHER = {Soci\'et\'e Math\'ematique de France (SMF), Paris},
    VOLUME = {47},
      YEAR = {1919},
     PAGES = {161--271},
 ZBLNUMBER = {47.0921.02},
       DOI = {10.24033/bsmf.998},
       URL = {http://www.numdam.org/item?id=BSMF_1919__47__161_0},
}



%% SOFTWARE

@manual{sagemath,
       KEY = {SageMath},
    AUTHOR = {{The Sage Developers}},
     TITLE = {{T}he {S}age {M}athematics {S}oftware {S}ystem ({V}ersion 8.1)},
      YEAR = {2017},
       URL = {http://www.sagemath.org},
}


@manual{Macaulay2,
       KEY = {M2},
    AUTHOR = {Grayson, D. and Stillman, M.},
     TITLE = {Macaulay2, a software system for research in algebraic geometry ({V}ersion 1.11)},
      YEAR = {2018},
       URL = {http://www.math.uiuc.edu/Macaulay2/},
}



%%% GitHub repository

@misc{GitHubRepo,
       KEY = {GitHub},
    AUTHOR = {Guillot, A. and Ramirez, V.},
     TITLE = {Multipliers-of-self-maps-on-{P}2},
 PUBLISHER = {GitHub},
HOWPUBLISHED = {GitHub repository. \url{https://github.com/valentermz/Multipliers-of-self-maps-on-P2}},
      NOTE = {2018},
}

